Evolving Differentiable Gene Regulatory Networks

Over the past twenty years, artificial Gene Regulatory Networks (GRNs) have shown their capacity to solve real-world problems in various domains such as agent control, signal processing and artificial life experiments. They have also benefited from new evolutionary approaches and improvements to dynamic which have increased their optimization efficiency. In this paper, we present an additional step toward their usability in machine learning applications. We detail an GPU-based implementation of differentiable GRNs, allowing for local optimization of GRN architectures with stochastic gradient descent (SGD). Using a standard machine learning dataset, we evaluate the ways in which evolution and SGD can be combined to further GRN optimization. We compare these approaches with neural network models trained by SGD and with support vector machines.

==> related.tex <==
%% \section{Background}
%% \label{sec:related}

Artificial GRNs were first proposed using a binary encoding of proteins with
specific start and stop codons, similar to biological genetic encoding
\cite{Banzhaf2003}. GRNs have since been used in a number of domains, including
robot control \cite{Joachimczak2010a}, signal processing \cite{Joachimczak2010},
wind farm design, \cite{Wilson2013}, and reinforcement learning
\cite{Cussat-Blanc2015}. Finding similar use to their biological inspiration,
GRNs have controlled the design and development of multi-cellular creatures
\cite{Cussat-Blanc2008} and of artificial neural networks (ANNs)
\cite{Wrobel2012}.

The performance of GRNs on these tasks has been improved by studies into both
the evolution and dynamics of GRNs. GRNEAT \cite{Cussat-Blanc2015a} takes after
the NEAT algorithm to increase GRN size over evolutionary time, to protect
genetic innovation using speciation, and to crossover similar genetic material.
A comparison of multiple GRN dynamics equations and encodings has shown that a
floating point encoding for GRNs can perform better than an integer encoding and
determining the best dynamics equations across various benchmarks
\cite{disset2017comparison}.

% From review paper
Artificial GRNs have been used to investigate a number of questions in the
context of evolution. Using Reil's DNA-like model \cite{Reil99}, Rohlf and
Winkler studied the evolvability of GRNs and showed a strong relationship
between their robustness against noise and their robustness against genetic
material deletions due to the evolutionary process \cite{rohlf_emergent_2009},
which are key properties in real-world applications. Schramm et al. investigated
the role of redundancy in artificial gene regulatory networks
\cite{schramm2012redundancy}, showing that genetic redundancy can enhance
evolvability up to a point, after which greater redundancy becomes deleterious.
Genetic networks were able to evolve modular genotypes when subjected to dynamic
fitness landscapes \cite{lipson_origin_2002}. Recent work has shown that evolved
GRNs can achieve greater hierarchical modularity than neural networks
\cite{lowell_developmental_2016}. Numerous studies remain to be performed
regarding the evolution of GRNs.

%% In this study, an ANN was evolved using an evolutionary fitness based on
%% performance after learning, which showed great improvement at the evolutionary
%% time scale, demonstrating the power of the Baldwin effect. The results of this
%% study are revisited and analyzed in \cite{santos2015phenotypic}, which argues
%% that the evolutionary methods in the original study could have reached similar
%% performance without learning. In \cite{gruau1993adding}, both the Baldwin effect
%% and Lamarckian evolution are studied in a developmental model of ANNs. In this
%% work, it was found that changing the fitness landscape using evolution, in other
%% words, the Baldwin effect, was as effective as passing on learned information to
%% offspring, Lamarckian evolution. While the results from both of these works are
%% significant, the models and problems used in both studies were restricted by
%% computational limits of the times and it is worth understanding if the same
%% conclusions can be drawn using more complex models and fitness landscapes.

%% In \cite{miikkulainen2017evolving}, Baldwinian evolution is used implicitly by
%% evolving the topology, components, and hyperparameters of deep neural network
%% architectures. The resulting architectures are comparable to those made by human
%% design. Both of these works demonstrate evolution's capability in a
%% computationally intensive domain, but aim more to prove this utility than to
%% illuminate the relationship between evolution and learning.

%% A high level overview of this relationship can be found in \cite{watson2016can},
%% which links learning theory to evolution theory.

The relationship between evolution and learning in artifical agents has a long
history of study. Although this study constitutes the first look at this
relationship using GRNs, ANNs have been used to understand both the Baldwin
effect and Lamarckian evolution. ANNs have been evolved with the option of
allowing certain weights to be learned, demonstrating that learning can improve
evolution's ability to reach difficult parts of the search space
\cite{hinton1987learning}. Lamarckian evolution has been used to combine
evolution of the structure of a Complex Pattern Producing Network and learning
of the network's weights \cite{fernando2016convolution}. This work intends to
explore the relationship between evolution and learning in the context of GRNs,
which are detailed next.


==> review.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  INTERNAL DYNAMICS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% FROM THE GRN REVIEW PAPER
\section{Internal dynamics of GRNs}
\label{sec:dynamics}

Before applying gene regulation to agent control, researchers have focused on the understanding on the internal dynamics of  gene regulation. In 1999,  Reil was one of the first to present a biologically plausible model used in an artificial life context \citep{Reil99}. In his work, he randomly generated a set of variable size binary genomes in which each gene started with the particular sequence 0101, named ``promoter''. Promoters exist in living systems: a very specific sequence of nucleotides, the $TATA$\footnote{$T$=Thymine and $A$=Adenine} box, is known to identify a gene's starting position. As presented in Fig. \ref{Rei_genes}, Reil used a simple visualization technique to observe gene activation and inhibition over time with randomly generated networks. He obtained several activation patterns such as stable, chaotic, or oscillatory patterns. Reil also pointed out that after random genome deteriorations, the system was able to rebuild the same pattern through an oscillation period.

\begin{figure}[h!]
\center
\setlength{\tabcolsep}{0.2mm}
\begin{tabular}{ccc}
\includegraphics[width=0.33\linewidth]{ReviewFigs/Rei_1.png} & 
\includegraphics[width=0.33\linewidth]{ReviewFigs/Rei_2.png} & 
\includegraphics[width=0.33\linewidth]{ReviewFigs/Rei_3.png} \\
(a) Ordered & (b) Chaotic & (c) Cyclic
\end{tabular}
\caption{Graphical representation of gene activation with Reil's artificial regulatory network. Each line represents one gene activation level: Dot means that the gene is activated; white space means it is disabled. Image from \citep{Reil99}.}\label{Rei_genes}
\end{figure}

The artificial gene regulatory network proposed in \citep{banzhaf_artificial_2003} is strongly inspired by real gene regulation. In this work, the genome is coded as a set of 32-bit integer (in other words a bit string). Each gene of a genome starts with a ``promoter'' coded by the sequence ``XYZ01010101'' where XYZ is any bit sequence to complete a 32-bit integer. The combination ``01010101'' has a probability of $2^{-8}$ in a bit string  equivalent to a TATA box from a real DNA sequence. The gene coded after a promoter has a fixed size of five integers (160 bits, each integer having 32 bits). Upstream from the promoter, two integers code for an enhancing site and for an inhibiting site, thus regulating gene expression activity. In this model, all DNA transcription mechanisms are omitted to focus on gene regulation dynamics itself. This kind of genome can produce various activation dynamics, as presented in Figure \ref{Banzhaf_ARN}. Randomly generated genomes were used in these experiments.

\begin{figure}[h!]
\center
\setlength{\tabcolsep}{0.2mm}
\begin{tabular}{ccc}
\includegraphics[width=0.33\linewidth]{ReviewFigs/banzhaf_1.jpg} & 
\includegraphics[width=0.33\linewidth]{ReviewFigs/banzhaf_2.jpg} & 
\includegraphics[width=0.33\linewidth]{ReviewFigs/banzhaf_3.jpg}
\end{tabular}
\caption{Examples of protein concentration dynamics obtained with the artificial gene regulatory network of \citep{banzhaf_artificial_2003}.}\label{Banzhaf_ARN}
\end{figure}

A key property observed in these networks is heterochrony \citep{banzhaf2003dynamics}. As depicted by Figure \ref{fig:heterochrony}, small changes in the network structure or concentration only imply small changes in network dynamics. This behavior is crucial when the network is evolved for artificial life applications: heterochrony smoothes the fitness landscape, making it more evolvable. This model has also been used in \citep{byrne_examination_2014} to analyze the inner temporal dynamics of gene regulatory networks using pole balancing and signal processing benchmarks and its capacity to reproduce input signals within a delayed timeframe.

\begin{figure}[h!]
\centering
\includegraphics[width=0.75\linewidth]{ReviewFigs/heterochrony.pdf}
\caption{Example of heterochronic control in gene regulatory networks: by mutating one bit of a protein, the regulation dynamics only slightly changed.}
\label{fig:heterochrony}
\end{figure}

Pictures and videos have been employed to visualize the dynamics of GRNs and observe the complexity of the behaviors generated. In a contribution by another author of this review \citep{Cussat-Blanc2012a} the GRN, cloned to every pixel of the picture, computed the RGB components of each pixel of the picture. Each GRN used the pixel coordinates (input proteins) to compute the color component (output proteins). GRNs were evolved using interactive evolution: users were tasked with selecting the most beautiful images, and GRNs were mutated and recombined based on this selection mechanism. Some of the generated pictures, representing a snapshot of the network dynamics, are presented in Fig. \ref{fig:GRNPictures}, while Fig. \ref{fig:GRNVideos} presents screenshots of videos\footnote{More examples and the software to generate pictures and videos can be found online: \url{http://www.irit.fr/~Sylvain.Cussat-Blanc/ColorfulRegulation/index_en.php}}. This work allowed to explore possible behavioral structures generated by gene regulatory networks. For example, in picture (b) of Fig. \ref{fig:GRNPictures}, repetitive patterns can be observed with some modifications. That shows the capacity of gene regulatory networks to produce modular patterns. Pictures (b-d) also show the ability of the GRN to produce both smooth or abrupt variation as codified here in color transitions. Finally, picture (e) depicts the GRN's capacity to produce extremely complex behavior, with very different outputs for close input values. More details about properties highlighted in these pictures can be found in \citep{Cussat-Blanc2012a}. 

Videos can capture the temporal aspect of gene regulation. As presented on Figure \ref{fig:GRNVideos}, oscillatory behaviors can be easily visualized. Other videos show chaotic and steady-state behaviors, which are the two other main behaviors of gene regulatory networks in addition to oscillations. 

\begin{figure}[t!]
\center
\setlength{\tabcolsep}{0.5mm}
\begin{tabular}{ccccc}
\includegraphics[width=0.195\linewidth]{ReviewFigs/GRNPicture_1.png} &
\includegraphics[width=0.195\linewidth]{ReviewFigs/GRNPicture_2.png} &
\includegraphics[width=0.195\linewidth]{ReviewFigs/GRNPicture_3.png} &
\includegraphics[width=0.195\linewidth]{ReviewFigs/GRNPicture_4.png} &
\includegraphics[width=0.195\linewidth]{ReviewFigs/GRNPicture_5.png} \\
(a) & (b) & (c) & (d) & (e)
\end{tabular}
\caption{Examples of pictures generated with a gene regulatory network. Image from \citep{Cussat-Blanc2012a}.}\label{fig:GRNPictures}
\end{figure}

\begin{figure}[t!]
\center
\includegraphics[width=\linewidth]{ReviewFigs/GRNVideo.png}
\caption{Examples of videos generated with a gene regulatory network.}\label{fig:GRNVideos}
\end{figure}

Artificial GRNs have been used to investigate a number of questions in the context of evolution. Using Reil's DNA-like model, Rohlf and Winkler studied the evolvability of GRNs and showed a strong relationship between their robustness against noise and their robustness against genetic material deletions due to the evolutionary process \citep{rohlf_emergent_2009}, which are key properties in real-world applications. Schramm et al. investigated the role of redundancy in artificial gene regulatory networks \citep{schramm2012redundancy}, showing that genetic redundancy can enhance evolvability up to a point, after which greater redundancy becomes deleterious. Genetic networks were able to evolve modular genotypes when subjected to dynamic fitness landscapes \citep{lipson_origin_2002}. Recent work has shown that evolved GRNs can achieve greater hierarchical modularity than neural networks \citep{lowell_developmental_2016}. Numerous studies remain to be performed regarding the evolution of GRNs, and some of those can be approached from the perspective of artificial life which is our next topic.

